Adjusted Objects: An Efficient and Principled Approach to Scalable Programming (Extended Version)

Parallel programs require software support to coordinate access to shared data. For this purpose, modern programming languages provide strongly-consistent shared objects. To account for their many usages, these objects offer a large API. However, in practice, each program calls only a tiny fraction of the interface. Leveraging such an observation, we propose to tailor a shared object for a specific usage. We call this principle adjusted objects. Adjusted objects already exist in the wild. This paper provides their first systematic study. We explain how everyday programmers already adjust common shared objects (such as queues, maps, and counters) for better performance. We present the formal foundations of adjusted objects using a new tool to characterize scalability, the indistinguishability graph. Leveraging this study, we introduce a library named DEGO to inject adjusted objects in a Java program. In micro-benchmarks, objects from the DEGO library improve the performance of standard JDK shared objects by up to two orders of magnitude. We also evaluate DEGO with a Retwis-like benchmark modeled after a social network application. On a modern server-class machine, DEGO boosts by up to 1.7x the performance of the benchmark.

==> Makefile <==
ALL=$(wildcard *.tex)
BIB=$(wildcard *.bib)
BIBTEX=bibtex
MAIN=main
LATEX=pdflatex

.DEFAULT_GOAL := all

rfast:
	@$(LATEX) $(MAIN).tex

bib:
	@$(BIBTEX) $(F).aux

all:
	@$(LATEX) $(MAIN).tex
	@$(BIBTEX) $(MAIN).aux
	@$(LATEX) $(MAIN).tex
	@$(LATEX) $(MAIN).tex

clean: ## Clean LaTeX and output figure files
	latexmk -c

arxiv:
	mkdir -p arxiv/
	cp acmart.cls arxiv/
	cp Makefile arxiv/
	cp format.sty arxiv/
	cp macros.sty arxiv/
	cp main.sty arxiv/
	cp pgf-pie.sty arxiv/
	cp abstract.tex arxiv/
	cp main.tex arxiv/
	cp introduction.tex arxiv/
	cp model.tex arxiv/
	cp distinguishability.tex arxiv/
	cp adjusted.tex arxiv/
	cp design.tex arxiv/
	cp evaluation.tex arxiv/
	cp related.tex arxiv/
	cp conclusion.tex arxiv/
	cp appendix/model.tex arxiv/appendix-model.tex
	sed -i -e s/{appendix\\/model/{appendix-model/g arxiv/main.tex 
	cp appendix/proofs.tex arxiv/appendix-proofs.tex
	sed -i -e s/{appendix\\/proofs/{appendix-proofs/g arxiv/main.tex
	cp figures/tree.tex arxiv/figures-tree.tex
	sed -i -e s/{figures\\/tree/{figures-tree/g arxiv/adjusted.tex
	cp figures/ref.tex arxiv/figures-ref.tex
	sed -i -e s/{figures\\/ref/{figures-ref/g arxiv/distinguishability.tex
	cp figures/set.tex arxiv/figures-set.tex
	sed -i -e s/{figures\\/set/{figures-set/g arxiv/distinguishability.tex
	cp figures/cnt.tex arxiv/figures-cnt.tex
	sed -i -e s/{figures\\/cnt/{figures-cnt/g arxiv/distinguishability.tex
	cp figures/spec.tex arxiv/figures-spec.tex
	sed -i -e s/{figures\\/spec/{figures-spec/g arxiv/distinguishability.tex
	cp figures/mining/evolution.tex arxiv/figures-mining-evolution.tex
	sed -i -e s/{figures\\/mining\\/evolution/{figures-mining-evolution/g arxiv/design.tex
	cp figures/mining/hotfiles.tex arxiv/figures-mining-hotfiles.tex
	sed -i -e s/{figures\\/mining\\/hotfiles/{figures-mining-hotfiles/g arxiv/design.tex
	cp figures/mining/distribution.tex arxiv/figures-mining-distribution.tex
	sed -i -e s/{figures\\/mining\\/distribution/{figures-mining-distribution/g arxiv/evaluation.tex
	cp figures/listings/AtomicWriteOnceReference.java arxiv/
	sed -i -e s/{figures\\/listings\\/AtomicWriteOnceReference.java/{AtomicWriteOnceReference.java/g arxiv/introduction.tex
	cp figures/AtomicLong_stack_graph.tex arxiv/figures-AtomicLong_stack_graph.tex
	sed -i -e s/{figures\\/AtomicLong_stack_graph/{figures-AtomicLong_stack_graph/g arxiv/introduction.tex
	cp figures/AtomicLong_cassandra_graph.tex arxiv/figures-AtomicLong_cassandra_graph.tex
	sed -i -e s/{figures\\/AtomicLong_cassandra_graph/{figures-AtomicLong_cassandra_graph/g arxiv/introduction.tex
	cp results/highcontention.tex arxiv/results-highcontention.tex
	sed -i -e s/{results\\/highcontention/{results-highcontention/g arxiv/evaluation.tex
	cp results/Counter/Counter.tex arxiv/results-counter-counter.tex
	sed -i -e s/{results\\/Counter\\/Counter/{results-counter-counter/g arxiv/results-highcontention.tex
	cp results/Map/HashMap.tex arxiv/results-map-hashmap.tex
	sed -i -e s/{results\\/Map\\/HashMap/{results-map-hashmap/g arxiv/results-highcontention.tex
	cp results/Map/SkipListMap.tex arxiv/results-map-skiplistmap.tex
	sed -i -e s/{results\\/Map\\/SkipListMap/{results-map-skiplistmap/g arxiv/results-highcontention.tex
	cp results/Reference/Reference.tex arxiv/results-reference-reference.tex
	sed -i -e s/{results\\/Reference\\/Reference/{results-reference-reference/g arxiv/results-highcontention.tex
	cp results/Queue/Queue.tex arxiv/results-queue-queue.tex
	sed -i -e s/{results\\/Queue\\/Queue/{results-queue-queue/g arxiv/results-highcontention.tex
	cp results/Map/ratio_write/mixedworkload.tex arxiv/results-mixedworkload.tex
	sed -i -e s/{results\\/Map\\/ratio_write\\/mixedworkload/{results-mixedworkload/g arxiv/evaluation.tex
	cp results/Map/ratio_write/25_update.tex arxiv/results-mixedworkload-25.tex
	sed -i -e s/{results\\/Map\\/ratio_write\\/25_update/{results-mixedworkload-25/g arxiv/results-mixedworkload.tex
	cp results/Map/ratio_write/50_update.tex arxiv/results-mixedworkload-50.tex
	sed -i -e s/{results\\/Map\\/ratio_write\\/50_update/{results-mixedworkload-50/g arxiv/results-mixedworkload.tex
	cp results/Map/ratio_write/75_update.tex arxiv/results-mixedworkload-75.tex
	sed -i -e s/{results\\/Map\\/ratio_write\\/75_update/{results-mixedworkload-75/g arxiv/results-mixedworkload.tex
	cp results/Map/ratio_write/100_update.tex arxiv/results-mixedworkload-100.tex
	sed -i -e s/{results\\/Map\\/ratio_write\\/100_update/{results-mixedworkload-100/g arxiv/results-mixedworkload.tex
	cp results/Map/sizes.tex arxiv/results-sizes.tex
	sed -i -e s/{results\\/Map\\/sizes/{results-sizes/g arxiv/evaluation.tex
	cp results/Retwis/results.tex arxiv/results-retwis-results.tex
	sed -i -e s/{results\\/Retwis\\/results/{results-retwis-results/g arxiv/evaluation.tex
	cp results/Retwis/alpha.tex arxiv/results-retwis-alpha.tex
	sed -i -e s/{results\\/Retwis\\/alpha/{results-retwis-alpha/g arxiv/evaluation.tex
	cp figures/power.tex arxiv/figures-power.tex
	sed -i -e s/{figures\\/power/{figures-power/g arxiv/appendix-proofs.tex
	cp biblio.bib arxiv/
	cp main.bbl arxiv/
	cp plainnat.bst arxiv/
	tar -C arxiv -zcf arxiv.tar.gz .
	rm -Rf arxiv/

watch: ## Recompile on any update of LaTeX or SVG sources
	@while [ 1 ]; do;          \
	  inotifywait $(ALL);    \
	  sleep 0.01;            \
          make all;              \
          echo "\n----------\n"; \
          done

help:  # http://marmelab.com/blog/2016/02/29/auto-documented-makefile.html
	@grep -P '^[a-zA-Z_-]+:.*?## .*$$' $(MAKEFILE_LIST) | sort | awk 'BEGIN {FS = ":.*?## "}; {printf "\033[36m%-20s\033[0m %s\n", $$1, $$

.PHONY: help



==> results-counter-counter.tex <==
\begin{axis}[
    ylabel={Kops/s per thread},
    xticklabels={1,5,10,20,40,80},
    xtick={1,2,3,4,5,6},
    xlabel={\# threads},
    ytick={0,10,1.0E2,1.0E3,1.0E4,1.0E5,1.0E6,1.0E7,1.0E8,1.0E9,1.0E10,1.0E11},
    extra y ticks={1},
    extra y tick labels={$0$},
    ymin=1,
    ymax=100000000,
    xmin=1,
    xmax=6,
    y=0.35cm,
    ymode=log,
    % xmode=log,
    % scale only axis,
    log origin=0,
    ymajorgrids,
    axis x line*=bottom,
    axis y line*=left,
    ylabel style={font=\Huge},
    xlabel style={font=\Huge},
    title style={font=\Huge},
    tick label style={font=\Huge},
    legend style={draw=none, at={(0.5,-0.3)}, anchor=north, font=\Huge},
    title=Counter]
    \addplot coordinates {
       (1, 154765.6395445897)
       (2, 5021.503156857267)
       (3, 2631.0593323767516)
       (4, 884.0981304780541)
       (5, 714.130981379835)
       (6, 295.8325283090249)
   };

    \addplot coordinates {
       (1, 277068.0611408808)
       (2, 248880.30558936112)
       (3, 244467.35383320638)
       (4, 200529.12050627964)
       (5, 104422.7448064383)
       (6, 103396.36587756606)
   };

    \addplot coordinates {
       (1, 124936.06569980961)
       (2, 115085.20681922624)
       (3, 108590.02301962413)
       (4, 89287.20050478342)
       (5, 63611.298689897405)
       (6, 63298.22967117156)
   };

  \legend{CounterJUC, CounterIncrementOnly, LongAdder, };
\end{axis}

==> results-map-hashmap.tex <==
\begin{axis}[
    % ylabel={KOp/s per process},
    xticklabels={1,5,10,20,40,80},
    xtick={1,2,3,4,5,6},
    % xlabel={\# threads},
    ytick={0,10,1.0E2,1.0E3,1.0E4,1.0E5,1.0E6,1.0E7,1.0E8,1.0E9,1.0E10,1.0E11},
    yticklabel={\empty},
    % extra y ticks={1},
    % extra y tick labels={$0$},
    ymin=1,
    ymax=100000000,
    xmin=1,
    xmax=6,
    y=0.35cm,
    ymode=log,
    % xmode=log,
    % scale only axis,
    log origin=0,
    ymajorgrids,
    axis x line*=bottom,
    axis y line*=left,
    ylabel style={font=\Huge},
    xlabel style={font=\Huge},
    title style={font=\Huge},
    tick label style={font=\Huge},
    legend style={draw=none, at={(0.5,-0.3)}, anchor=north,font=\Huge},
    title=HashMap]
    \addplot coordinates {
       (1, 28859.235163162775)
       (2, 13219.57877477844)
       (3, 10053.318590921393)
       (4, 7742.145958822342)
       (5, 4950.976427528401)
       (6, 1548.2763277142435)
   };
    \addplot coordinates {
       (1, 45903.597819691364)
       (2, 37935.72655601506)
       (3, 37241.41307259667)
       (4, 28060.711331207316)
       (5, 17766.151117597743)
       (6, 6871.250201747607)
   };
  \legend{ConcurrentHashMap, ExtendedSegmentedHashMap, };
\end{axis}

==> results-map-skiplistmap.tex <==
\begin{axis}[
    % ylabel={KOp/s per process},
    xticklabels={1,5,10,20,40,80},
    xtick={1,2,3,4,5,6},
    % xlabel={\# threads},
    ytick={0,10,1.0E2,1.0E3,1.0E4,1.0E5,1.0E6,1.0E7,1.0E8,1.0E9,1.0E10,1.0E11},
    yticklabel={\empty},
    % extra y ticks={1},
    % extra y tick labels={$0$},
    ymin=1,
    ymax=100000000,
    xmin=1,
    xmax=6,
    y=0.35cm,
    ymode=log,
    % xmode=log,
    % scale only axis,
    log origin=0,
    ymajorgrids,
    axis x line*=bottom,
    axis y line*=left,
    ylabel style={font=\Huge},
    xlabel style={font=\Huge},
    title style={font=\Huge},
    tick label style={font=\Huge},
    legend style={draw=none, at={(0.5,-0.3)}, anchor=north,font=\Huge},
    title=SkipListMap]
    \addplot coordinates {
       (1, 5487.682525891692)
       (2, 3443.4520762244492)
       (3, 2921.001392264968)
       (4, 2243.1849142607443)
       (5, 1525.7872605107796)
       (6, 795.3959857673584)
   };
    \addplot coordinates {
       (1, 7412.112587931876)
       (2, 6565.543027612203)
       (3, 6154.133896060591)
       (4, 4933.434046232254)
       (5, 2643.349149302537)
       (6, 785.1901435131768)
   };
  \legend{ConcurrentSkipListMap, ExtendedSegmentedSkipListMap, };
\end{axis}

==> results-mixedworkload-100.tex <==
\begin{axis}[
ybar,
width=0.275\linewidth,
height=0.25\textwidth,
bar width=0.01\linewidth,
ylabel={100\% upd},
ytick={0, 1.0E4, 2.0E4, 3.0E4, 4.0E4, 5.0E4, 6.0E4, 7.0E4, 8.0E4, 9.0E4, 1.0E5},
yticklabel={\empty},
ymin=0,
ymax=100000,
symbolic x coords={LeftMargin, Unordered, Space, Ordered, RightMargin},
ymajorgrids,
axis x line*=bottom,
axis y line*=left,
xtick=data,
legend style={draw=none, at={(0.5,1.2)}, anchor=north},
xmin=LeftMargin,
xmax=RightMargin,
ylabel style={font=\footnotesize},
xlabel style={font=\footnotesize},
title style={font=\footnotesize},
tick label style={font=\footnotesize},
cycle list={ {fill=orange}, {fill=orange} },
area legend,
scaled y ticks=false,]
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,45903) +- (2423, 2422) 
 (Ordered,7411) +-(166, 166) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,37935) +- (820, 819) 
 (Ordered,6565) +-(224, 223) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,37240) +- (1422, 1423) 
 (Ordered,6153) +-(48, 49) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,28060) +- (805, 804) 
 (Ordered,4932) +-(59, 60) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,17765) +- (794, 794) 
 (Ordered,2642) +-(6, 6) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,6870) +- (175, 176) 
 (Ordered,784) +-(11, 11) };
% \legend{DEG}
\end{axis}

\begin{axis}[
ybar,
width=0.275\linewidth,
height=0.25\textwidth,
bar width=0.01\linewidth,
% ylabel={75\% upd},
ytick={0, 1.0E4, 2.0E4, 3.0E4, 4.0E4, 5.0E4, 6.0E4, 7.0E4, 8.0E4, 9.0E4, 1.0E5},
ymin=0,
ymax=100000,
symbolic x coords={LeftMargin, Unordered, Space, Ordered, RightMargin},
ylabel style={font=\footnotesize},
xlabel style={font=\footnotesize},
title style={font=\footnotesize},
tick label style={font=\footnotesize},
% ymajorgrids,
axis lines=none,
xtick=data,
legend style={draw=none, at={(0.5,1.1)}, anchor=north},
xmin=LeftMargin,
xmax=RightMargin,
cycle list={ {fill=RoyalBlue!90!white}, {fill=RoyalBlue!90!white} },
area legend,
yticklabel={\empty},
xticklabel={\empty},
scaled y ticks=false,]
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,28858) +- (57, 57) 
 (Ordered,5487) +-(118, 118) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,13219) +- (139, 139) 
 (Ordered,3443) +-(56, 55) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,10053) +- (116, 115) 
 (Ordered,2920) +-(34, 34) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,7741) +- (43, 43) 
 (Ordered,2242) +-(35, 35) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,4950) +- (36, 36) 
 (Ordered,1525) +-(16, 15) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,1547) +- (18, 18) 
 (Ordered,794) +-(10, 11) };
% \legend{JUC}
\end{axis}

==> results-mixedworkload-25.tex <==
\begin{axis}[
ybar,
width=0.275\linewidth,
height=0.25\textwidth,
bar width=0.01\linewidth,
ylabel={\shortstack{25\% upd \\ Kops/s per thread}},
ytick={0, 1.0E4, 2.0E4, 3.0E4, 4.0E4, 5.0E4, 6.0E4, 7.0E4, 8.0E4, 9.0E4, 1.0E5},
ymin=0,
ymax=100000,
symbolic x coords={LeftMargin, Unordered, Space, Ordered, RightMargin},
ymajorgrids,
axis x line*=bottom,
axis y line*=left,
xtick=data,
legend style={draw=none, at={(0.8,1)}, anchor=north, font=\footnotesize},
xmin=LeftMargin,
xmax=RightMargin,
ylabel style={font=\footnotesize},
xlabel style={font=\footnotesize},
title style={font=\footnotesize},
y tick label style={font=\footnotesize},
x tick label style={font=\footnotesize},
cycle list={ {fill=orange}, {fill=orange} },area legend,]

\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=6pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,75361) +- (497, 498) [1]
(Ordered,10326) +- (266, 266)
};
 
\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=7pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,47527) +- (4399, 4399) [5]
(Ordered,9793) +- (62, 62)
};
 
\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=9pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,41890) +- (3635, 3634) [10]
(Ordered,9101) +- (117, 117)
};
 
\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=6pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,39622) +- (3215, 3216) [20]
(Ordered,7228) +- (165, 165)
};
 
\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=6pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,27171) +- (881, 881) [40]
(Ordered,5057) +- (66, 65)
};
 
\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=6pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,18851) +- (1313, 1313) [80]
(Ordered,3926) +- (142, 142)
};
 
\legend{\sys}
\end{axis}

\begin{axis}[
ybar,
width=0.275\linewidth,
height=0.25\textwidth,
bar width=0.01\linewidth,
% ylabel={\shortstack{25\% upd \\ Kops/s per thread}},
ytick={0, 1.0E4, 2.0E4, 3.0E4, 4.0E4, 5.0E4, 6.0E4, 7.0E4, 8.0E4, 9.0E4, 1.0E5},
ymin=0,
ymax=100000,
symbolic x coords={LeftMargin, Unordered, Space, Ordered, RightMargin},
% ymajorgrids,
axis lines=none,
xtick=data,
xticklabel style={/pgf/number format/.cd, fixed},
legend style={draw=none, at={(0.77,0.85)}, anchor=north, font=\footnotesize},
xmin=LeftMargin,
xmax=RightMargin,
ylabel style={font=\footnotesize},
xlabel style={font=\footnotesize},
title style={font=\footnotesize},
tick label style={font=\footnotesize},
cycle list={ {fill=RoyalBlue!90!white}, {fill=RoyalBlue!90!white} },
area legend,
yticklabel={\empty},
xticklabel={\empty}]

\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=6pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,64642) +- (438, 437) 
(Ordered,5095) +- (35, 35)
 };
 
\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=6pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,39054) +- (102, 102) 
(Ordered,3795) +- (25, 25)
};
 
\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=6pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,31364) +- (113, 113) 
(Ordered,3162) +- (20, 19)
};
 
\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=6pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,21114) +- (224, 223) 
(Ordered,2356) +- (14, 15)
};
 
\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=6pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,11166) +- (58, 57) 
(Ordered,1556) +- (11, 12)
};
 
\addplot+[nodes near coords, point meta=explicit symbolic, every node near coord/.append style={yshift=6pt, xshift=-0.1cm, rotate=45, anchor=west, font=\footnotesize}, error bars/.cd, y dir=both, y explicit] coordinates {
(Unordered,2159) +- (62, 63) 
(Ordered,1141) +- (16, 15)
};
\legend{JUC}
\end{axis}

==> results-mixedworkload-50.tex <==
\begin{axis}[
ybar,
width=0.275\linewidth,
height=0.25\textwidth,
bar width=0.01\linewidth,
ylabel={50\% upd},
ytick={0, 1.0E4, 2.0E4, 3.0E4, 4.0E4, 5.0E4, 6.0E4, 7.0E4, 8.0E4, 9.0E4, 1.0E5},
yticklabel={\empty},
ymin=0,
ymax=100000,
symbolic x coords={LeftMargin, Unordered, Space, Ordered, RightMargin},
ymajorgrids,
axis x line*=bottom,
axis y line*=left,
xtick=data,
legend style={draw=none, at={(0.8,1.3)}, anchor=north, font=\footnotesize},
xmin=LeftMargin,
xmax=RightMargin,
ylabel style={font=\footnotesize},
xlabel style={font=\footnotesize},
title style={font=\footnotesize},
tick label style={font=\footnotesize},
cycle list={ {fill=orange}, {fill=orange} },
area legend,
scaled y ticks=false,
]
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,67828) +- (1189, 1188) 
 (Ordered,9483) +-(48, 49) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,39561) +- (5625, 5625) 
 (Ordered,8470) +-(117, 118) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,37534) +- (5181, 5181) 
 (Ordered,7709) +-(202, 202) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,29881) +- (3300, 3299) 
 (Ordered,6158) +-(203, 203) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,22455) +- (744, 743) 
 (Ordered,4051) +-(132, 132) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,13149) +- (611, 611) 
 (Ordered,2336) +-(75, 75) };
% \legend{DEG}
\end{axis}

\begin{axis}[
ybar,
width=0.275\linewidth,
height=0.25\textwidth,
bar width=0.01\linewidth,
% ylabel={50\% upd},
% ytick={0, 1.0E4, 2.0E4, 3.0E4, 4.0E4, 5.0E4, 6.0E4, 7.0E4, 8.0E4, 9.0E4, 1.0E5},
ymin=0,
ymax=100000,
symbolic x coords={LeftMargin, Unordered, Space, Ordered, RightMargin},
% ymajorgrids,
axis lines=none,
xtick=data,
legend style={draw=none, at={(0.9,1.2)}, anchor=north},
xmin=LeftMargin,
xmax=RightMargin,
ylabel style={font=\footnotesize},
xlabel style={font=\footnotesize},
title style={font=\footnotesize},
tick label style={font=\footnotesize},
cycle list={ {fill=RoyalBlue!90!white}, {fill=RoyalBlue!90!white} },
area legend,
yticklabel={\empty},
xticklabel={\empty},
scaled y ticks=false,]
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,49032) +- (357, 356) 
 (Ordered,4579) +-(37, 36) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,26612) +- (109, 109) 
 (Ordered,3187) +-(19, 19) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,20520) +- (194, 194) 
 (Ordered,2682) +-(12, 13) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,12712) +- (141, 140) 
 (Ordered,2015) +-(10, 11) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,6328) +- (72, 71) 
 (Ordered,1363) +-(5, 6) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,1005) +- (28, 28) 
 (Ordered,923) +-(7, 7) };
% \legend{JUC}
\end{axis}

==> results-mixedworkload-75.tex <==
\begin{axis}[
ybar,
width=0.275\linewidth,
height=0.25\textwidth,
bar width=0.01\linewidth,
ylabel={75\% upd},
ytick={0, 1.0E4, 2.0E4, 3.0E4, 4.0E4, 5.0E4, 6.0E4, 7.0E4, 8.0E4, 9.0E4, 1.0E5},
yticklabel={\empty},
ymin=0,
ymax=100000,
symbolic x coords={LeftMargin, Unordered, Space, Ordered, RightMargin},
ymajorgrids,
axis x line*=bottom,
axis y line*=left,
xtick=data,
legend style={draw=none, at={(0.5,1.2)}, anchor=north,font=\footnotesize},
xmin=LeftMargin,
xmax=RightMargin,
ylabel style={font=\footnotesize},
xlabel style={font=\footnotesize},
title style={font=\footnotesize},
tick label style={font=\footnotesize},
cycle list={ {fill=orange}, {fill=orange} },
area legend,
scaled y ticks=false,]
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,64885) +- (1228, 1228) 
 (Ordered,8624) +-(55, 55) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,32700) +- (8584, 8584) 
 (Ordered,7646) +-(180, 181) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,36599) +- (6005, 6005) 
 (Ordered,7016) +-(239, 239) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,25137) +- (4618, 4618) 
 (Ordered,5328) +-(325, 325) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,19609) +- (2219, 2219) 
 (Ordered,3350) +-(163, 163) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,9859) +- (548, 548) 
 (Ordered,1672) +-(81, 80) };
% \legend{DEG}
\end{axis}

\begin{axis}[
ybar,
width=0.275\linewidth,
height=0.25\textwidth,
bar width=0.01\linewidth,
% ylabel={75\% upd},
ytick={0, 1.0E4, 2.0E4, 3.0E4, 4.0E4, 5.0E4, 6.0E4, 7.0E4, 8.0E4, 9.0E4, 1.0E5},
ymin=0,
ymax=100000,
symbolic x coords={LeftMargin, Unordered, Space, Ordered, RightMargin},
% ymajorgrids,
axis lines=none,
xtick=data,
legend style={draw=none, at={(0.1,1.3)}, anchor=north,font=\footnotesize},
xmin=LeftMargin,
xmax=RightMargin,
ylabel style={font=\footnotesize},
xlabel style={font=\footnotesize},
title style={font=\footnotesize},
tick label style={font=\footnotesize},
cycle list={ {fill=RoyalBlue!90!white}, {fill=RoyalBlue!90!white} },
area legend,
yticklabel={\empty},
xticklabel={\empty},
scaled y ticks=false,]
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,41426) +- (318, 317) 
 (Ordered,4279) +-(37, 38) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,21030) +- (64, 64) 
 (Ordered,2817) +-(37, 36) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,15584) +- (214, 215) 
 (Ordered,2355) +-(18, 19) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,8959) +- (492, 492) 
 (Ordered,1793) +-(9, 10) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,4459) +- (67, 68) 
 (Ordered,1205) +-(11, 12) };
\addplot+[error bars/.cd, y dir=both, y explicit] coordinates {(Unordered,689) +- (44, 44) 
 (Ordered,777) +-(9, 9) };
% \legend{JUC}
\end{axis}

==> results-queue-queue.tex <==
\begin{axis}[
    xticklabels={2,5,10,20,40,80},
    xtick={1,2,3,4,5,6},
    % xlabel={\# threads},
    ytick={0,10,1.0E2,1.0E3,1.0E4,1.0E5,1.0E6,1.0E7,1.0E8,1.0E9,1.0E10,1.0E11},
    yticklabel={\empty},
    % extra y ticks={1},
    % extra y tick labels={$0$},
    ymin=1,
    ymax=100000000,
    xmin=1,
    xmax=6,
    y=0.35cm,
    ymode=log,
    % xmode=log,
    % scale only axis,
    log origin=0,
    ymajorgrids,
    axis x line*=bottom,
    axis y line*=left,
    ylabel style={font=\Huge},
    xlabel style={font=\Huge},
    title style={font=\Huge},
    tick label style={font=\Huge},
    legend style={draw=none, at={(0.5,-0.3)}, anchor=north, font=\Huge},
    title=Queue]
    \addplot coordinates {
       (1, 51677.52686736793)
       (2, 1715.6201267122997)
       (3, 670.8677005220344)
       (4, 187.4440935774715)
       (5, 165.90487351868626)
       (6, 32.2560968101899)
   };

    \addplot coordinates {
       (1, 60754.72545288924)
       (2 9606.417875982095)
       (3, 2628.430320460143)
       (4, 764.6759218118157)
       (5, 707.5020129667148)
       (6, 221.10206546847945)
   };

  \legend{ConcurrentLinkedQueue, QueueMASP, };
\end{axis}

==> results-reference-reference.tex <==
\begin{axis}[
    % ylabel={KOp/s per process},
    xticklabels={1,5,10,20,40,80},
    xtick={1,2,3,4,5,6},
    % xlabel={\# threads},
    ytick={0,10,1.0E2,1.0E3,1.0E4,1.0E5,1.0E6,1.0E7,1.0E8,1.0E9,1.0E10,1.0E11},
    yticklabel={\empty},
    % extra y ticks={1},
    % extra y tick labels={$0$},
    ymin=1,
    ymax=100000000,
    xmin=1,
    xmax=6,
    y=0.35cm,
    ymode=log,
    % xmode=log,
    % scale only axis,
    log origin=0,
    ymajorgrids,
    axis x line*=bottom,
    axis y line*=left,
    ylabel style={font=\Huge},
    xlabel style={font=\Huge},
    title style={font=\Huge},
    tick label style={font=\Huge},
    legend style={draw=none, at={(0.5,-0.3)}, anchor=north, font=\Huge},
    title=Reference]
    \addplot coordinates {
       (1, 1444365.6955562294)
       (2, 1317148.673390407)
       (3, 1229100.6323083122)
       (4, 982759.9931800934)
       (5, 577341.1683187163)
       (6, 544650.3930521674)
   };

    \addplot coordinates {
       (1, 28106892.431392174)
       (2, 18916983.795898404)
       (3, 17337890.048944604)
       (4, 12244962.23135723)
       (5, 2982710.9367347853)
       (6, 1840635.357423238)
   };

  \legend{AtomicReference, AtomicWriteOnceReference, };
\end{axis}
